Near-Optimal Multi-Agent Learning for Safe Coverage Control

In multi-agent coverage control problems, agents navigate their environment to reach locations that maximize the coverage of some density. In practice, the density is rarely known $\textit{a priori}$, further complicating the original NP-hard problem. Moreover, in many applications, agents cannot visit arbitrary locations due to $\textit{a priori}$ unknown safety constraints. In this paper, we aim to efficiently learn the density to approximately solve the coverage problem while preserving the agents' safety. We first propose a conditionally linear submodular coverage function that facilitates theoretical analysis. Utilizing this structure, we develop MacOpt, a novel algorithm that efficiently trades off the exploration-exploitation dilemma due to partial observability, and show that it achieves sublinear regret. Next, we extend results on single-agent safe exploration to our multi-agent setting and propose SafeMac for safe coverage and exploration. We analyze SafeMac and give first of its kind results: near optimal coverage in finite time while provably guaranteeing safety. We extensively evaluate our algorithms on synthetic and real problems, including a bio-diversity monitoring task under safety constraints, where SafeMac outperforms competing methods.

==> extra-text-neurips.tex <==

Please read the instructions below carefully and follow them faithfully.


\subsection{Style}


Papers to be submitted to NeurIPS 2022 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2022 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2022.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2022 is \verb+neurips_2022.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2022.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2022+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2022}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}


\section{Final instructions}


Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2022/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> extra/algo.tex <==
%By definition the operator is mutually exclusive, i.e, the resulting collection has a property that $\forall~\batch_1,\batch_2 \in \BatchColl{t}, \batch_1 \neq \batch_2, \batch_1 \cap \batch_2 = \emptyset$ and also, $\sum_{\batch \in \BatchColl{t}} |\batch| = \numOfAgents$.

% The \safemac runs \macopt(compute \greedy solution) for each $\batch \in \BatchColl{t}$ in the restricted region defined by $\uniSet[,B]{t} \coloneqq \cup_{i \in \batch} \uniSet[,i]{t}$. \greedy algorithm returns a set of disk centers, which are guaranteed to be either in the optimistic or in the pessimistic set and are potentially good locations to maximize coverage. 


%\safemac now has a coverage goal based on the optimistic coverage value on an optimistically safe domain. Now \safemac applies the disk operator at these locations and identifies the location of maximum information below the disks, and sets them as a goal-to-go (\cref{alg: max-density-width-under-disk}). If the goal-to-go locations are within their $\pessiSet[, i]{t}$, the agents request the density measurement and get its noisy observation (\cref{alg: density-meas}). The agents share this observation with all the other agents and update their posterior beliefs based on the gathered data (\cref{alg: density-gp-update}). Based on the updated belief over $\density$, it recomputes a new location for coverage maximization (\cref{alg: new-greedy}). On the other hand if the set-goal-to-go are not in the pessimistic set but in $\optiSet[,i]{t}\backslash \pessiSet[,i]{t}$, then \safemac deploys \goose's goal directed safe expansion module (\cref{alg: SE-module-st}-\ref{alg: SE-module-end}).

% is a multi-agent instantiation of \goose. For every agent $i$, \safemac deploy \goose to maintain two sets: a pessimistic safe set and an optimistic safe set. The pessimistic safe set  contains the states that are safe with high probability and is necessary to guarantee safe exploration \citep{turchetta2019safe}. The pessimistic set will stay the same or increase in size with every set update operation. In contrast, the optimistic set will stay the same or generally shrink as the agents identify unsafe regions. After some time $t$, it is possible that the agents have a disconnected optimistic set. 

% \textbf{Batching operation} at any time t, will group the agents together which lies in an optimistically safely connected region and possibly will maximize the coverage jointly with the greedy strategy. For our setup of $\numOfAgents$ agents, the collection of batches $\BatchColl{t} \coloneqq \BatchColl{t}([\numOfAgents])$ operator is defined as,
% \begin{align*}
%   \BatchColl{t} = \bigcup_{i \in [\numOfAgents]} \BatchColl{t}'(i)~~\textit{where}~~\BatchColl{t}'(i) &= \{ j \in [\numOfAgents] \, | \, \uniSet[,i]{t} \cap \uniSet[,j]{t} \neq \emptyset \}, ~~\textit{and}~~ \uniSet[,i]{t} \coloneqq \optiSet[,i]{t} \cup \pessiSet[,i]{t}.    \numberthis \label{eqn: uni-batching}
% \end{align*}
% With the above operation we have partitioned agents into batches, such that for any batch $\batch \in \BatchColl{t}$ contains the agents which are topologically connected in either their pessimistic or optimistic set or both (\cref{alg: batching}). By definition the operator is mutually exclusive, i.e, the resulting collection has a property that $\forall~\batch_1,\batch_2 \in \BatchColl{t}, \batch_1 \neq \batch_2, \batch_1 \cap \batch_2 = \emptyset$ and also, $\sum_{\batch \in \BatchColl{t}} |\batch| = \numOfAgents$.

% \textbf{Optimistic \macopt} 

% The \safemac algorithm runs in two phases \textit{optimistic coverage phase} (\cref{alg: coverage-phase}) and the \textit{optimistic exploration phase} (\cref{alg: exploration-phase}). Both the phases are coupled but differ in the goal-to-go for the agents. In the coverage phase agent safely explores in the direction of potential coverage maximizers where as in the exploration phase agent explores $\constrain(\PtInDomain)$ below the placed disk. The agents do not need to explore the whole domain in the exploration phase but only the potentially good coverage locations. In \safemac, both the phases alternate as per the requirement and the collected samples.

% \todo{May be this para is not so useful}
% Let us start first with the optimistic coverage phase. Like \macopt, the agents solve a \greedy algorithm and receive the location to place the disk (\cref{alg: init-greedy}). In the coverage phase, we set goal-to-go as the locations under the respective disks conditioned on the previous disk below every agent. In contrast to \macopt, in the constrained case, since the environment is \textit{a-priori} unknown, we do not know if the goal-to-go is safe or not. Each agent does safe exploration in the direction of goal-to-go using the safe expansion module of \goose.

% \mypar{Multi-agent \goose} 
% is a multi-agent instantiation of \goose. For every agent $i$, \safemac deploy \goose to maintain two sets: a pessimistic safe set and an optimistic safe set. The pessimistic safe set  contains the states that are safe with high probability and is necessary to guarantee safe exploration \citep{turchetta2019safe}. The pessimistic set will stay the same or increase in size with every set update operation. In contrast, the optimistic set will stay the same or generally shrink as the agents identify unsafe regions. After some time $t$, it is possible that the agents have a disconnected optimistic set. Since the coverage problem is inherently a cooperative task, where multiple agents jointly maximize a common objective, \safemac has to know about the agents that are optimistically together but disconnected from the rest so that they can locally maximize coverage.

% \textbf{Batching operation} at any time t, will group the agents together which lies in an optimistically safely connected region and possibly will maximize the coverage jointly with the greedy strategy. For our setup of $\numOfAgents$ agents, the collection of batches $\BatchColl{t} \coloneqq \BatchColl{t}([\numOfAgents])$ operator is defined as,
% \begin{align*}
%   \BatchColl{t} = \bigcup_{i \in [\numOfAgents]} \BatchColl{t}'(i)~~\textit{where}~~\BatchColl{t}'(i) &= \{ j \in [\numOfAgents] \, | \, \uniSet[,i]{t} \cap \uniSet[,j]{t} \neq \emptyset \}, ~~\textit{and}~~ \uniSet[,i]{t} \coloneqq \optiSet[,i]{t} \cup \pessiSet[,i]{t}.    \numberthis \label{eqn: uni-batching}
% \end{align*}
% With the above operation we have partitioned agents into batches, such that for any batch $\batch \in \BatchColl{t}$ contains the agents which are topologically connected in either their pessimistic or optimistic set or both (\cref{alg: batching}). By definition the operator is mutually exclusive, i.e, the resulting collection has a property that $\forall~\batch_1,\batch_2 \in \BatchColl{t}, \batch_1 \neq \batch_2, \batch_1 \cap \batch_2 = \emptyset$ and also, $\sum_{\batch \in \BatchColl{t}} |\batch| = \numOfAgents$.

% \textbf{Optimistic \macopt} Next, \safemac runs \macopt(compute \greedy solution) for each $\batch \in \BatchColl{t}$, on the domain defined by $\uniSet[,B]{t} \coloneqq \cup_{i \in \batch} \uniSet[,i]{t}$. \greedy algorithm returns a set of disk centers, which are guaranteed to be either in the optimistic or in the pessimistic set and are potentially good locations to maximize coverage. \safemac now has a coverage goal based on the optimistic coverage value on an optimistically safe domain. Now \safemac applies the disk operator at these locations and identifies the location of maximum information below the disks, and sets them as a goal-to-go (\cref{alg: max-density-width-under-disk}). If the goal-to-go locations are within their $\pessiSet[, i]{t}$, the agents request the density measurement and get its noisy observation (\cref{alg: density-meas}). The agents share this observation with all the other agents and update their posterior beliefs based on the gathered data (\cref{alg: density-gp-update}). Based on the updated belief over $\density$, it recomputes a new location for coverage maximization (\cref{alg: new-greedy}). On the other hand if the set-goal-to-go are not in the pessimistic set but in $\optiSet[,i]{t}\backslash \pessiSet[,i]{t}$, then \safemac deploys \goose's goal directed safe expansion module (\cref{alg: SE-module-st}-\ref{alg: SE-module-end}).

==> extra/analysis.tex <==
% In practice, the algorithm is terminated as per stopping criteria of achieving $\epsdensity$ accurate coverage. For this, the immediate corollary of the above theorem is,
% \begin{corollary}
% Let $\tdensity^{\star}$ be the smallest integer, such that $\frac{\tdensity^{\star}}{\beta_{\tdensity^{\star}} \gamma_{K\tdensity^{\star}}} \leq \frac{8 K^2 }{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}$, then there exists a $t < \tdensity^{\star}$ such that with probability $1-\delta$, \macopt terminates and achieves, 
% \begin{align*}
%     \Objfunc{\LocAgents_{t}}{\density}{\Domain} \geq (1- \frac{1}{e}) \Objfunc{\LocAgents_{\star}}{\density}{\Domain} - \epsilon_{\density}
% \end{align*}
% \end{corollary}
% The corollary says that at each round, if we build hypothetical disks as per \greedy UCB and observe max uncertain points within the discs, then we are guaranteed a near optimal coverage up to $\epsdensity$ accurate in a finite time.

% Could we maybe shrink this down to a remark that just says that it is easy to show that once the stopping criterion is met it is easy to show we are within \epsilon from the lower bound of the greedy solution? This would save a lot of space and we could give a forward reference to the appendix












%We can directly say we bound the slot wise regret with the information capacity, a quantity that measures the largest reduction in uncertainty about the density that can be obtained from KT noisy evaluations of it.
% % First is the greedy selection for the constraint submodular maximization \citep{Nemhauser-1minus1by-e}. 

% % Along with this, we exploit the conditional linearity of the objective function (\cref{eqn: disk-coverage}) and bound the cumulative regret defined in \cref{eqn: reg-def} with a surrogate regret. 
% % The surrogate regret decouples the joint regret in \cref{eqn: reg-def} to a sum of $\numOfAgents$ independent per agent regret. 

% Second is the upper confidence bounds of \GP \citep{beta-srinivas}. 









% We bound the per agent's regret with the accumulated information $I(y_A | \density)$, where $A$ is the set of observations collected as per \macopt ($\cref{alg:greedyUCB:selection}$).  




% To bound the regret, we need to quantify the information \macopt can acquire through the noisy density observations. Any subset $A$ of observations $y_A = \{ y_i | i \in A\}$, reduces our uncertainty about the density $\density$.




% The proof for Theorem 1 is in \cref{Apx: thm-macopt}. The proof build on two key ideas, greedy selection for the constraint submodular maximization and upper confidence bounds of \GP. First we exploit the conditional linearity of the objective function (\cref{eqn: disk-coverage}), and bound the cumulative regret defined in \cref{eqn: reg-def} with a surrogate regret. The surrogate regret decouples the joint regret to a sum of $\numOfAgents$ independent per agent regret. Next, we bound the per agent regret with the accumulated information $I(y_A | \density)$, where $A$ is the set of observations collected as per \macopt ($\cref{alg:greedyUCB:selection}$). 

% upper bounds the regret of sampling at the upper confidence of coverage function instead of the true coverage. 

% we build an upper confidence bound on the coverage function using $\updensity[t]$ instead of true $\density$ with appropriate $\betadensity[T]$ \citep{beta-chowdhury17a}. Further, 

% This theorem guarantees that the recommendation will have a simple regret that converges at the sublinear rate in time on average. 

% In practice, the algorithm is terminated as per stopping criteria of achieving $\epsdensity$ accurate coverage. For this, the immediate corollary of the above theorem is,
% \begin{corollary}
% Let $\tdensity^{\star}$ be the smallest integer, such that $\frac{\tdensity^{\star}}{\beta_{\tdensity^{\star}} \gamma_{K\tdensity^{\star}}} \leq \frac{8 K^2 }{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}$, then there exists a $t < \tdensity^{\star}$ such that with probability $1-\delta$, \macopt terminates and achieves, 
% \begin{align*}
%     \Objfunc{\LocAgents_{t}}{\density}{\Domain} \geq (1- \frac{1}{e}) \Objfunc{\LocAgents_{\star}}{\density}{\Domain} - \epsilon_{\density}
% \end{align*}
% \end{corollary}
% The corollary says that at each round, if we build hypothetical disks as per \greedy UCB and observe max uncertain points within the discs, then we are guaranteed a near optimal coverage up to $\epsdensity$ accurate in a finite time.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%Premature recommend%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Pre-mature recommendation} If the algorithm is terminated at T, pre-matured before the stopping criteria we can recommend based on the following criteria,
% \begin{align*}
%     \LocAgents_T = \argmax_{\LocAgents_t \in \LocAgents_{1:T}}  \Objfunc{\LocAgents_t}{\lbdensity[t-1]}{\Domain} 
% \end{align*}
% where $\LocAgents_{1:T}$ is the set of all the greedy solution indexed at time $t \leq T$. For the above recommendation rule at time T, we show that the recommendation converges with $\mathcal{O}^{\star}(\sqrt{\frac{1}{T}})$. In particular, it holds with high probability that $(1- \frac{1}{e}) \Objfunc{\LocAgents_{\star}}{\density}{\Domain} - \Objfunc{\LocAgents_{T}}{\density}{\Domain}  < \mathcal{O}^{\star}(\numOfAgents \sqrt{\frac{\gammadensity{\numOfAgents T}}{T}})$.


%%%%%%%%%%%%%%%%%%%%%%Insert algorithm


% is met condition stopped at any time, we can still certify that the coverage is at least $\Obj(X_{t};\lbdensity[t], \Domain )$. 




% At every round t the algorithm picks $\numOfAgents$ locations greedily conditioning on the previously picked agents (Line 8).  


% The coverage maximization can be interpreted as an instance of partial monitoring, where maximization of coverage is decoupled from maximizing the utility function. We have to maximize coverage based on the partial information in the from the noisy utility measurements.   

% In this setting, the agents are well aware of the underlying domain. In the domain, they coordinate among themselves to identify the locations to collect measurement, keeping in perspective the best locations to maximize coverage.
% The agents here faces a two-tier of exploration-exploitation dilemma. Firstly the agent needs to learn about the density, and take decisions in order to maximize the coverage. 


% \manish{Greedy selection, UCB, max uncertain pt, partial information}\\


% We can note that the disk coverage function exhibit a conditional linear dependence on the $\density$. We will exploit this to derive an efficient algorithm. We can interpret it as partial monitoring where the agent explores to receive partial information of the coverage and finally exploit to maximize coverage based on the partial information.
% A natural strategy to balance the exploration and exploitation is to optimize coverage based on UCB of $\density$, essentially $\Obj(\LocAgents; \updensity, \Domain)$,

% However this rule is still too greedy and stucks in local optima due to partial information of the coverage. \macopt proposes to identify the location of "importance" as per UCB rule in order to minimize cummulative regret but collect observation at the locations of maximum uncertainty under the discs conditioned on the previous discs, given by,
% \begin{align*}
%   \LocAgent[m, i]{t} \leftarrow \argmax_{x \in \Discat[i]_t \backslash \Discat[1:i-1]_t} w^\density_t(x) 
% \end{align*}
% Using this 2 step acquisition rule, \macopt is not required to reduce the uncertainty everywhere in the domain but only at the coverage locations of interest defined by the utility function. 



% At every round t the algorithm picks $\numOfAgents$ locations greedily conditioning on the previously picked agents (Line 8).  

% \begin{corollary}
% For any $t \geq 1$, if $\sum_i^{\numOfAgents} 2 \sqrt{\beta_{t}} \max_{x \in \Discat[i]_t \backslash \Discat[1:i-1]_t} \sigma_{\density_{t -1}}(x) \leq \epsdensity$ the following holds,
% \begin{align*}
%     \Objfunc{X_{t}}{\density}{\Domain} \geq (1- \frac{1}{e}) \Objfunc{X^{\star}}{\density}{\Domain} - \epsilon_{\density}
% \end{align*}

% For any $T_{\epsdensity}$, the time when $\sum_i^{\numOfAgents} 2 \sqrt{\beta_{t}} \max_{x \in \Discat[i]_t \backslash \Discat[1:i-1]_t} \sigma_{\density_{t -1}}(x) \leq \epsdensity$ for the first time or "when the algorithm terminates", is bounded by:
% \begin{align*}
%     \frac{T_{\epsdensity}}{\beta_{T_{\epsdensity}} \gamma_{KT_{\epsdensity}}} \leq \frac{8 K^2 }{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}
% \end{align*}
% \end{corollary}



% \begin{algorithm}[!ht]
% \caption{\macopt}
% % \SetAlgoLined
% \begin{algorithmic}[1]
% \State \textbf{Inputs} Initial States / set $\LocAgents_0=[\LocAgent[1]{0},\LocAgent[2]{0}, . . . ,\LocAgent[k]{0}]$\\
% Graph $G$, Accuracy $\epsdensity$, Domain $\Domain$, $GP_{\density}(\mu^{\density}_{0}, k^{\density})$
% \State \textbf{Initialize} $t \leftarrow 0$, $W^m_0 = \infty$
% \State $\LocAgent[1:k]{t} \leftarrow $ GreedyUCBsolution($GP_{\density}, \Domain$)
% \While{$W^m_t \geq \epsilon_{\density}$}  \manish{Note that this $W^m_t$ is of the next round} 
% \State $\forall i \in [\numOfAgents]$, $\LocAgent[m, i]{t} \leftarrow \argmax_{x \in \Discat[i]_t \backslash \Discat[1:i-1]_t} w^\density_t(x) $
% \State $\forall i \in [\numOfAgents]$, observe $y^i_{\density_t} = \density(\LocAgent[m,i]{t}) + \noise_{\density}$
% \State $t \leftarrow t + 1$
% \State $\LocAgent[1:k]{t} \leftarrow $ GreedyUCBsolution($GP_{\density}, \Domain$)
% \State $ W^m_t \leftarrow \sum_{i}^{\numOfAgents} \max_{x \in \Discat[i]_t \backslash \Discat[1:i-1]_t} w^\density_t(x)$
% \EndWhile
% \State \textbf{Recommend:} $\LocAgents_t$
% \end{algorithmic}
% \end{algorithm}


% , we receive noisy observations of unknown $\density$ model.
% \noindent\usebox{\algleft}\hfill\usebox{\algright}%
% Since the underlying safe exploration algo makes

==> extra/appx-safemac.tex <==
We know that when cumulative regret over time after $\tdensity^{n-1}$ is less than $\epsdensity$, then at least once $r_t\leq\epsdensity$ after $\tdensity^{n-1}$. We want upper bound of \eq~\ref{eqn: t2-eps-bound} over $\deltime{2}$ to be less than $\epsdensity$, this gives,
    \begin{align*} \sqrt{ \frac{8 \numOfAgents^2 \betadensity[\tdensity^{1} + \deltime{2}] I(Y_{\deltime{2}};\density) }{\deltime{2}\log(1+\numOfAgents\sigma^{-2})}} \leq \epsdensity
    \end{align*}
    Similar to \lem~\ref{lem: const-time-bound}, we get bound on $\deltime{2}$ \todo{add a lemma similar to lemma 12 here}
    \begin{align*}
        \frac{\deltime{2}}{\betadensity[\tdensity^{1} + \deltime{2}] I(Y_{\deltime{2}};\density)} &\geq \frac{8 K^2 }{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}
    \end{align*}
So there exists $\smdeltime{2} < \deltime{2}$, such that $r_t \leq \epsdensity$ after $\tdensity^{1}$.
% ~\manish{Issues with equalities, might be we have to add + 1, every time \macopt converges}
% Consider $\tdensity^{1} + \deltime{2}$,

\todo{add a lemma for recursively adding up time n times}
Let ${\tdensity^{\star}}^{2} \geq \tdensity^{1} + \smdeltime{2}$ and the smallest integer satisfying $\frac{{\tdensity^{\star}}^{2}}{ \betadensity[{\tdensity^{\star}}{2}] \gammadensity{\numOfAgents {\tdensity^{\star}}^{2}}} \geq \frac{8 K^2}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}$. There exists a time $\tdensity^{2} \in [\tdensity^{1}, {\tdensity^{\star}}^{2}]$ such that \macopt stopping criteria is satisfied $\sumMaxWidth{t}\leq\epsdensity$.
\begin{itemize}
    \item After $\tdensity^{1} + \deltime{2}$ density measurements, we check again i.e. $\uncertaindisk = \emptyset$,  if not then we evaluate $\deltime{3}$, $\deltime{4}$, so and so forth
\end{itemize}
% Let say \macopt stopping criteria is satisfied for the $nth$ time, we know that,
% \begin{align*}
%     \tdensity^{n} &\leq \tdensity^{1} + \deltime{2} + \deltime{3} \hdots +\deltime{n} \\
%     &\leq \frac{8 K^2 \betadensity[\tdensity^{1}] I(Y_{\LocAgent[g,1:\numOfAgents]{1:\tdensity^{1}}};\density)}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2} + \frac{8 K^2 \betadensity[\tdensity^{1} + \deltime{2}] I(Y_{\deltime{2}};\density)}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2} + \hdots + \frac{8 K^2 \betadensity[\tdensity^{n-1} + \deltime{n}] I(Y_{\deltime{n}};\density)}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}  \tag{using \eq~\ref{eqn: t1-bound}} \\
%     &\leq \frac{8 K^2 \betadensity[\tdensity^{n-1} + \deltime{n}]}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}( I(Y_{\LocAgent[g,1:\numOfAgents]{1:\tdensity^{1}}};\density) +  I(Y_{\deltime{2}};\density) + \hdots +I(Y_{\deltime{n}};\density)) \tag{Since, $\betadensity[t]$ is non decreasing function} \\
%     &= \frac{8 K^2 \betadensity[\tdensity^{n-1} + \deltime{n}]}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}( I(Y_{\LocAgent[g,1:\numOfAgents]{1:\tdensity^{n-1} + \deltime{n}}};\density)  
% \end{align*}
    % \begin{align*}
    %     \tdensity^{1} + \deltime{2} &\geq \tdensity^{1} + \frac{8 K^2 \betadensity[\tdensity^{1} + \deltime{2}] I(Y_{\deltime{2}};\density)}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2} \\
    %     \tdensity^{1} + \deltime{2} &\geq \frac{8 K^2 \betadensity[\tdensity^{1}] I(Y_{\LocAgent[g,1:\numOfAgents]{1:\tdensity^{1}}};\density)}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2} + \frac{8 K^2 \betadensity[\tdensity^{1} + \deltime{2}] I(Y_{\deltime{2}};\density)}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2} \tag{using \eq~\ref{eqn: t1-bound}}\\
    %     \tdensity^{1} + \deltime{2} &\geq \frac{8 K^2 }{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}(\betadensity[\tdensity^{1}] I(Y_{\LocAgent[g,1:\numOfAgents]{1:\tdensity^{1}}};\density) + \betadensity[\tdensity^{1} + \deltime{2}] I(Y_{\deltime{2}};\density)) \\ \tag{Since, $\betadensity[t]$ is non decreasing function} \\
    %     \tdensity^{1} + \deltime{2} &\geq \frac{8 K^2 }{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}(\betadensity[\tdensity^{1} + \deltime{2}] I(Y_{\LocAgent[g,1:\numOfAgents]{1:\tdensity^{1} + \deltime{2}}};\density)) \numberthis \label{eqn: t2-bound} \\
    %     % &\leq \frac{8 K^2 \betadensity[\tdensity^{1} + \deltime{2}] \gammadensity{\numOfAgents \tdensity^{1} + \deltime{2}} }{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2} \tag{At any time  $=\tdensity^{1} + \deltime{2}$, we can bound mutual with $\gamma$}
    % \end{align*}

        \manish{Does the computation of $\tdensity^{1}$ and $\tdensity^{1} + \deltime{2}$ makes sense? It is bit counter intuitive that even if \safemac converges after $\tdensity^{n}$ the bound says that $\tdensity^{n} < {\tdensity^{\star}}^{n}$ where ${\tdensity^{\star}}^{n}$ is the smallest integer satisfying $\frac{{\tdensity^{\star}}^{n}}{ \betadensity[{\tdensity^{\star}}^{n}] \gammadensity{\numOfAgents {\tdensity^{\star}}^{n}}} \geq \frac{8 K^2}{ \log(1+\numOfAgents\sigma^{-2}) \epsdensity^2}$. If we think of it in reverse direction, that is if we have reached time $\tdensity^{\star}$ that would mean that there is no uncertain region below the disk. Since both the GP's $(\density, \constrain)$ are separate, this conclusion sounds weird. } % That means we don't lose anything even if \macopt converges multiple time and it is the same bound even if you run \safemac on the fully explored environment (2 stage case).}
\begin{itemize}
    \item In the worst case the algorithm can go until $\optiSet[, i]{t}  \subseteq \pessiSet[, i]{t}, \forall i \in [\numOfAgents]$ that is, we need to explore the whole domain, after this anyways $(\optiSet[]{t} \cap \Discat[1:\numOfAgents]_t) \subseteq (\pessiSet[]{t} \cap \Discat[1:\numOfAgents]_t)$. Hence our result will follow. 
    \item Goose says that $\optiSet[,i]{t}  \subseteq \pessiSet[,i]{t} $ will happen in a finite time.
\end{itemize}

==> extra/coverage.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%Coverage function%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Coverage function}
The disk coverage function $\Obj: 2^{\Domain} \times \Domain \times 2^{\Domain} \to \R$ in a connected set $\Domain$ is given by,
\begin{align*}
\Objfunc{A}{\density}{\Domain} = \sum_{\PtInDomain \in \Domain} \density(\PtInDomain) \min \Big \{ \frac{\intThresh}{\factor}, \sum_{\LocAgent[i]{} \in A} \diskcover(\LocAgent[i]{} , \PtInDomain) \Big\}  \numberthis %\label{eqn: disk-coverage}
\end{align*}
where $\intThresh$ is an integer. We used $\intThresh=1$ in this work and $\diskcover(\LocAgent[i]{} , \PtInDomain)$ is coverage of location $\PtInDomain$ by agent located at $\LocAgent[i]{}$, formally given by,
\begin{align*}
\diskcover(\LocAgent[i]{} , \PtInDomain) = \begin{cases} \frac{1}{\factor} & \text{if } \PtInDomain \in \Discat[i] \\
0 & \text{if } \PtInDomain \notin \Discat[i]
\end{cases} 
% We can think of X_i as a disk(set) centered around x_i.
% A = {1,2, ..... n}, let c'(A, \PtInDomain) = min{\intThresh, \sum_{i \in A} c(X_i , \PtInDomain)}. The coverage of \PtInDomain under A.
% The function f with f(A) = \sum{A \in \Domain} c'(A, \PtInDomain) is sub modular.
\end{align*}
where, $\Discat[i]:= \Roperator{Disc}{}{\LocAgent[i]{t}} := \Domain \cap \Roperator{Reach, \diskradius}{}{\LocAgent[i]{t}}$, denoting a disk or a patch in which the agent can reach in the $\diskradius$ steps and N is the maximum number of nodes possible in the patch $\Discat[i]$ for any agent $i$. A patch is representative of the area, an agent is capable of covering based on it's sensing, dynamics and acting capabilities.\\

\textbf{Key property:} For any 2 disconnected domain $\Domain_1$ and $\Domain_2$, such that $\Domain_1 \cup \Domain_2 \subseteq \Domain$ and $A_1 \cup A_2 = A$, then,
\begin{align*}
    \Objfunc{A}{\density}{\Domain} = \Objfunc{A_1}{\density}{\Domain_1} + \Objfunc{A_2}{\density}{\Domain_2}
\end{align*}
We define the maximum achievable objective as:
\begin{align*}
    \sum_{\batch \in \BatchColl{r}} \Objfunc{\LocAgents^{\batch}_{\star}}{\density}{\Rbareps{}{\LocAgents^{\batch}_0}} 
\end{align*}
\textbf{Short notations:} $\Obj(.) := \Objfunc{.}{\density}{\Domain}$, that is if the utility $\density$ and the domain $\Domain$ are clear from the context as true utility $\density$ and complete domain $\Domain$, we will drop in notation for clarity.\\
With the abuse of notation we represent, $\Objfunc{\LocAgents_{\star}}{\density}{\Domain}:= \sum_{\batch \in \BatchColl{r}} \Objfunc{\LocAgents^{\batch}_{\star}}{\density}{\Rbareps{}{\LocAgents^{\batch}_0}}$. IMP point to note that the agents $\LocAgents_{\star}$ are constrained to be within there $\Rbareps{}{\LocAgents^{\batch}_0}$.

==> extra/glossary.tex <==
\usepackage[acronym,nomain]{glossaries}              % use glossaries-package


\setlength{\glsdescwidth}{15cm}

\newglossary[slg]{symbolslist}{syi}{syg}{Symbolslist} % create add. symbolslist

\makeglossaries                                   % activate glossaries-package

% ==== EXEMPLARY ENTRY FOR SYMBOLS LIST =========================================
    \newglossaryentry{symb:Pi}{name=\ensuremath{\pi},
        description={Geometrical value},
        type=symbolslist}

    \newglossaryentry{height}{name=\ensuremath{h},
        description={Height of tower},
        type=symbolslist}

    \newglossaryentry{energyconsump}{name=\ensuremath{P},
        description={Energy consumption},
        type=symbolslist}

\newglossarystyle{notationlong}{%
\setglossarystyle{long}% base this style on the list style
\renewenvironment{theglossary}{% Change the table type --> 3 columns
  \begin{longtable}{lp{0.6\glsdescwidth}}}%
  {\end{longtable}}%

\renewcommand*{\glossaryheader}{%  Change the table header
  \bfseries Sign & \bfseries Description \\
 \hline
  \endhead}
\renewcommand*{\glossentry}[2]{%  Change the displayed items
  \glstarget{##1}{\glossentryname{##1}} %
  & \glossentrydesc{##1}
  \tabularnewline
}

}




% \glsaddall

==> extra/optimistic_edge_oper.tex <==
We denote with $\edges{A}$, the edges from the set $\edges{}$ which connects nodes in set $A$, precisely,
\begin{align*}
    \edges{A} = \{ (x, z) \in \edges{}, | x \in A , z \in A\}
\end{align*}
Modification to the reachbility operator:
\begin{align*}
    \Roperator{reach}{}{S; \edges{A}} &= S \cup \{ \xDeci \in \D \backslash S, | \exists \zDeci \in S: (\zDeci,\xDeci) \in \edges{A} \},  \\
    \Roperator{reach,n}{}{S; \edges{A}} &= \Roperator{reach,n}{\edges{A}}{\Roperator{reach,n-1}{}{S; \edges{A}}} ~\text{with}~ \Roperator{reach,1}{}{S; \edges{A}} = \Roperator{reach}{}{S; \edges{A}} \\
    \Rtiloperator{reach}{}{S; \edges{A}} &= \lim_{n \to \infty}\Roperator{reach,n}{}{S; \edges{A}},
\end{align*}
% We define the union operator to update each agent's pessimistic set as:     
% \begin{align*}
%     \pessiSet[,i]{t+1} &= \Rtiloperator{reach}{}{\pessiSet[,i]{t}; \edges{\pessiSet[]{t}}^{1:\numOfAgents}},  \numberthis \label{eqn: pessi-update-operator} \\
%     \textit{where},~ \edges{\pessiSet[]{t}}^{1:\numOfAgents} &= \bigcup_{i=1}^{\numOfAgents} \edges{\pessiSet[,i]{t}} \neq \edges{\bigcup_{i=1}^{\numOfAgents} \pessiSet[,i]{t}}
% \end{align*}
We define the intersection operator of the optimistic set as:
\begin{align*}
    \optiSet[,i]{t+1} &= \Rtiloperator{reach}{}{\LocAgent[i]{0}; \edges{\optiSet[]{t}}^{1:\numOfAgents}}, \numberthis \label{eqn: opti-update-operator} \\
    \textit{where},~ \edges{\optiSet[]{t}}^{1:\numOfAgents} &= \edges{\D} - \bigcup_{i=1}^{\numOfAgents} \edges{\D} - (\edges{\optiSet[,i]{t}} \cup \edges{\D - \optiSet[,i]{t}})  \tag{Note that we did not start with $\pessiSet[,i]{t}$ but $\LocAgent[i]{0}$}
    % \edges{\pessiSet[]{t}}^{1:\numOfAgents} &= \bigcup_{i=1}^{\numOfAgents} \edges{\pessiSet[,i]{t}} \neq \edges{\bigcup_{i=1}^{\numOfAgents} \pessiSet[,i]{t}}
\end{align*}
The idea is that no 2 optimistic set should have any node in common. If they have anything in common then it's exactly same optimistic set. \todo{Prove the above statement. Also prove the shrinkage of this optimistic intersection operator.}
% \manish{$\Rtiloperator{reach}{}{\pessiSet[,i]{t}; \edges{\optiSet[]{t}}^{1:\numOfAgents}}$, probably i should start with $\LocAgents_0$ instead of pessimistic set.}\\
% \manish{Is it possible that the optimistic set has a disconnected region inside it? Since optimistic set start building from the pessimistic set, it might be the case that pessimistic set have point in the middle where $u<\epsilon$ THen the formed optimistic set from the pessimictic set will have disconnected region.}

==> extra/todo.tex <==
\section{ToDo}
\begin{itemize}
    \item \manish{this}
    \item \matteo{that}
\end{itemize}

==> sections/pts-to-think.tex <==


\subsection{IN PRELIMINARIES}

\begin{itemize}
    \item The unknown environment is modelled using a finite, deterministic $\MDP$.
    \item reward, density, 
\end{itemize}
\textbf{Coverage Objective:}
\begin{itemize}
    \item Disk coverage formulation
    \item truncated disk
\end{itemize}


$\Reachable$ is the maximum safely reachable set when the agents start at $\LocAgents_0$.

\textbf{Submodularity:}
Maybe Submodularity can be entirely addressed in the intro, related works.
\begin{itemize}
    \item 1 line definition of sub modularity
    \item Explain diminishing return, a lemma that above coverage is submodular
    \item NP-hard with agents<\numOfAgents
    \item Near-optimal solution in polynomial time
\end{itemize}

\textbf{Bayesian Optimization/Kernalized bandits/Regularity:}
\begin{itemize}
    \item lipschitz continuty 
    \item 
\end{itemize}

\textbf{Safe exploration}

\textbf{Goal}
\begin{itemize}
    \item Explain observation model
    \item path observation
    \item Regret definition
    \item Single point: near-optimal simple regret
    \item constraint case: talk about finite time
\end{itemize}


1. Compare with $1-1/e F(X^{*})$ vs $\sum_{i=1}^{\numOfAgents} \delgain{x_t|X_t^{1:i-1}}{\density}{\Rbar-eps}$                 
2. Compare with $F(X^{greedy}; \Rbar)$ vs $\sum_{i=1}^{\numOfAgents} \delgain{x_t|X_t^{1:i-1}}{\density}{\Rbar}$
3. compare with $\sum_{i=1}^{\numOfAgents} \delgain{\tilde{x}|X_t^{1:i-1}}{\density}{\optiSet}$ - $\delgain{x_t|X_t^{1:i-1}}{\density}{\optiSet}$
4. compare with $\sum_{i=1}^{\numOfAgents} \delgain{\tilde{x}|X_t^{1:i-1}}{\density}{\pessiSet}$ - $\delgain{x_t|X_t^{1:i-1}}{\density}{\pessiSet}$

We can compare with the first one and report the termination time. But it's not a right metric since we might be doing good in pessimistic set which is out of R bar, we can probably compare in Rbar0. The problem with this method is that the baseline suggested by andreas will actually be the best since 1-1/e is really a low number

2. Here if we do bad or worse wrt to F(X^greedy) doesn't mean that we are doing bad or good. It will be that case that you are performing poor with F(X^greedy) by converged faster. Comparing 2 greedy solution might not be the best idea

4. we can do this but tha algorithm is not designed for it.


The main reason is that we cannot compare 2 greedy solutions, one could be bad just how the domain looks like. 

